Retrieval Augmented Generation and Understanding in Vision: A Survey and New Outlook

Retrieval-augmented generation (RAG) has emerged as a pivotal technique in artificial intelligence (AI), particularly in enhancing the capabilities of large language models (LLMs) by enabling access to external, reliable, and up-to-date knowledge sources. In the context of AI-Generated Content (AIGC), RAG has proven invaluable by augmenting model outputs with supplementary, relevant information, thus improving their quality. Recently, the potential of RAG has extended beyond natural language processing, with emerging methods integrating retrieval-augmented strategies into the computer vision (CV) domain. These approaches aim to address the limitations of relying solely on internal model knowledge by incorporating authoritative external knowledge bases, thereby improving both the understanding and generation capabilities of vision models. This survey provides a comprehensive review of the current state of retrieval-augmented techniques in CV, focusing on two main areas: (I) visual understanding and (II) visual generation. In the realm of visual understanding, we systematically review tasks ranging from basic image recognition to complex applications such as medical report generation and multimodal question answering. For visual content generation, we examine the application of RAG in tasks related to image, video, and 3D generation. Furthermore, we explore recent advancements in RAG for embodied AI, with a particular focus on applications in planning, task execution, multimodal perception, interaction, and specialized domains. Given that the integration of retrieval-augmented techniques in CV is still in its early stages, we also highlight the key limitations of current approaches and propose future research directions to drive the development of this promising area.

==> config.tex <==
\usepackage{amsmath}
\usepackage{tabularx}

\newcommand{\wrt}{\text{w.r.t.}}

==> figures/1_article_tree.tex <==
\tikzstyle{my-box}=[
    rectangle,
    rounded corners,
    text opacity=1,
    draw=black,
    minimum height=1em,
    minimum width=4em,
    inner sep=1pt,
    align=center,
    fill opacity=0,
]

\tikzstyle{cause_leaf}=[my-box, text=black, fill=blue!20, align=left, font=\scriptsize,
    inner xsep=3pt,
    inner ysep=3pt,
]

\tikzstyle{detect_leaf}=[my-box, text=black, fill=green!20, align=left, font=\scriptsize,
    inner xsep=3pt,
    inner ysep=3pt,
]

\tikzstyle{mitigate_leaf}=[my-box, text=black, fill=yellow!20, align=left, font=\scriptsize,
    inner xsep=3pt,
    inner ysep=3pt,
]

\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\scriptsize,
                draw=black,
                rectangle,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={black, line width=0.8pt},
                s sep=2pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{fill=blue!20, text width=4em, font=\scriptsize,}{},
            where level=2{fill=green!20, text width=6em, font=\scriptsize,}{},
            where level=3{fill=yellow!20, text width=6em, font=\scriptsize,}{},
            where level=4{fill=orange!20, text width=6em, font=\scriptsize,}{},
            [
            RAG for Computer Vision, ver, text=black
                [
                Understanding, text=black
                    [
                    Image Understanding, text=black
                        [
                        Recognition, text=black
                            [
                            Recognition, text=black
                                [\scriptsize{\textit{e.g.} RAC~\cite{long2022retrieval}}]
                            ]
                            [
                            Detection, text=black
                                [\scriptsize{\textit{e.g.} RALF~\cite{kim2024retrieval}}]
                            ]
                        ]
                        [
                        Image Captioning, text=black
                            [
                            Image-based, text=black
                                [\scriptsize{\textit{e.g.} SACO~\cite{zhou2023style}}]
                            ]
                            [
                            Caption-based, text=black
                                [\scriptsize{\textit{e.g.} EVCAP~\cite{li2024evcap}}]
                            ]
                            [
                            Image and Caption, text=black
                                [\scriptsize{\textit{e.g.} EXTRA~\cite{ramos2023retrieval}}]
                            ]
                        ]
                    ]
                    [
                    Video Understanding, text=black
                        [Understanding
                            , text=black
                                [\scriptsize{\textit{e.g.} VideoRAG~\cite{jeong2025videorag}}]
                        ]
                        [Long Video
                            , text=black
                                [\scriptsize{\textit{e.g.} Video-RAG~\cite{luo2024video}}]
                        ]
                        [Applications
                            , text=black
                            [\scriptsize{\textit{e.g.} Animate-A-Story~\cite{he2023animate}}]
                        ]
                    ]
                    [
                    Multi-modal, text=black
                        [
                        VQA, text=black
                            [
                            Multi-modal DB, text=black
                                [\scriptsize{\textit{e.g.} MuRAG~\cite{chen2022murag}}]
                            ]
                            [
                            Single-modal DB, text=black
                                [\scriptsize{\textit{e.g.} FLMR~\cite{lin2023finegrained}}]
                            ]
                        ]
                        [
                        Documents VQA, text=black
                            [
                            MLLMs, text=black
                                [\scriptsize{\textit{e.g.} ColPali~\cite{faysse2024colpali}}]
                            ]
                            [
                            OCR, text=black
                                [\scriptsize{\textit{e.g.} RAGFlow~\cite{ragflow}}]
                            ]
                        ]
                        [
                        Multi-task, text=black
                            [\scriptsize{\textit{e.g.} REACT~\cite{liu2023learning}}]
                        ]
                        [
                        Medical, text=black
                            [
                            Factuality, text=black
                                [\scriptsize{\textit{e.g.} MMED-RAG~\cite{xia2024mmed}}]
                            ]
                            [
                            Balance, text=black
                                [\scriptsize{\textit{e.g.} RULE~\cite{xia2024rule}}]
                            ]
                        ]
                    ]
                ]
                [
                Generation, text=black
                    [
                    Image Generation, text=black
                        [
                        Text-based, text=black
                            [\scriptsize{\textit{e.g.} DoFaiR~\cite{wan2024factuality}}]
                        ]
                        [
                        Vision-based, text=black
                            [\scriptsize{\textit{e.g.} RealRAG~\cite{lyu2024unibind}}]
                        ]
                    ]
                    [
                    Video Generation, text=black
                        [\scriptsize{\textit{e.g.} Animate-AS~\cite{he2023animate}}]
                    ]
                    [
                    3D Generation, text=black
                        [
                        Inference-based, text=black
                            [\scriptsize{\textit{e.g.} Phidias~\cite{wang2024phidias}}]
                        ]
                        [
                        Optimization-based, text=black
                            [\scriptsize{\textit{e.g.} ReDream~\cite{seo2024retrieval}}]
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{The main content flow and categorization of this survey.}
    \label{fig:categorization_of_survey}
\end{figure*}

